Inference from Auction Prices

Econometric inference allows an analyst to back out the values of agents in a mechanism from the rules of the mechanism and bids of the agents. This paper gives an algorithm to solve the problem of inferring the values of agents in a dominant-strategy mechanism from the social choice function implemented by the mechanism and the per-unit prices paid by the agents (the agent bids are not observed). For single-dimensional agents, this inference problem is a multi-dimensional inversion of the payment identity and is feasible only if the payment identity is uniquely invertible. The inversion is unique for single-unit proportional weights social choice functions (common, for example, in bandwidth allocation); and its inverse can be found efficiently. This inversion is not unique for social choice functions that exhibit complementarities. Of independent interest, we extend a result of Rosen (1965), that the Nash equilbria of "concave games" are unique and pure, to an alternative notion of concavity based on Gale and Nikaido (1965).

==> a_invtechext.tex <==

\section{Technical Extensions of Bid Inversion for Various Value Spaces}
\label{a:invtechext}






\subsection{Alternate Settings of Value Space and Weights Functions}

In the main body of the paper, we make the following assumptions to avoid ambiguity in the analysis:
\begin{itemize}
\item value space is $\left[0,H\right]^n$;
\item weights functions for all agents $i$ have $\wali(0) > 0$.
\end{itemize}

In this section we consider alternate assumptions for thoroughness, and to show general robustness against the assumptions of the main sections.  In turn we will consider:

\begin{enumerate}
\item value space again as $\left[0,H\right]^n$, but with weights functions for all agents $i$ having $\wali(0) = 0$;
\item (full version) value space as $\left(0,\infty\right)^n$ and $\wali(0) \geq 0$;
\item (full version) value space as $\left[\epsilon,H\right]^n$ and $\wali(0)\geq 0$.
\end{enumerate}

Of course, for (2) and (3), either strict positivity or non-negativity assumptions on weights functions at $\vali=0$ result in all value types having strictly positive weight, following from all value types in these settings are strictly positive and strict monotonicity of the weights functions.  These analyses are relegated to the full version of the paper.

The presentation of each setting contains a contextual discussion of the technical challenges introduced by the assumptions on value space and weights functions as applicable.

\subsubsection{Agents with Value 0 Participate and Get 0 Allocation}
\label{a:generalmech}

The setting is: value space as $\left[0,H\right]^n$, weights functions for all agents $i$ having $\wali(0) = 0$.

The first problem with this setting is that the ``simple" bid function is undefined at $\vali = \wali = 0$ (from equation~\eqref{eqn:bidfn:w}):
	\begin{equation*}
	\payi(\wals)=\vali(\wali)-\frac{\int^{\wali}_{\wali(0)}\alloci(z,\walsmi)\vali'(z)dz}{
    \alloci(\wals)}
	\end{equation*}
    
The problem is that we need to include $\wali = 0$ to get a closed domain space for $\pays$ to guarantee the existence of Nash in the proxy game.  Resolving this is non-trivial.

The \textit{winner-pays-bid bid-inversion mechanism} of definition~\ref{d:nash-mech} in Section~\ref{s:nasheq} assumes the bid function and its partials are well-defined such that they can be converted into a Rosen concave game.  Attempts to argue the necessity of $\strati(0) = 0$ from the requirements of equilibrium under the mechanism fail from begging the question- they depend on the class of equilibria which are possible given the mechanism, but the mechanism depends intrinsically on the bid function, for which it is our goal here to make sure it is well-defined.


However, we will be able to instead ``bootstrap" the same result.  A mechanism is simply an algorithmic computation.  Therefore, initially only for the purposes of computation within the mechanism, we can technically complete the definition of the bid function at $\wali=0$ by choice (as the designer).  The mechanism can use the \textit{internal} definition of the bid function- which is explicitly well-defined- for its computation.  Then the mechanism induces specific behavior in the agents in any equilibria, in particular at $\wali=0$ and we can make arguments about behavior here.  Finally we can formally prove that in the auction, that $\strati(0) = 0$ for this case, and go on to prove that the agents' play corresponds exactly to the computation already being performed by the mechanism.  In the end, we have implemented a technical design trick of the mechanism to let us choose and guarantee the agent behavior as $\strati(0) = 0$, which is a weakly dominant and natural action for the agents in the first place.

To be explicit and avoid ambiguity, we formally re-define the social choice function and the mechanism for this section~\ref{a:generalmech}.




The social choice function to be implemented is
\begin{equation*}
\alloci(\vali, \valsmi) = \frac{\wali(\vali)}{\wali[0]+\sum_{k\in\left\{1,...n\right\}}\wali[k](\vali[k])}
\end{equation*}
where $\wali[0] > 0$ is a constant weight added to the total in particular to guarantee continuity of the social choice function for all weights functions of our setting (continuous, differentiable, strictly increasing, $\wali(0)\geq 0$), and in general to make the allocation quantity $\alloci$ well-defined by avoiding \#div-0 errors.

The mechanism will define the following \textit{bid-smooth} function $\strati^{\delta}$ to use internally for its computations:
\begin{equation}
	\strati^{\delta}(\wals)\vcentcolon= \lim_{\delta\rightarrow 0} \left[\vali(\wali+\delta)-\frac{\int^{\wali+\delta}_{\wali(0)}\alloci(z,\walsmi)\vali'(z)dz}{
    \alloci(\wali+\delta,\walsmi)}\right]
\end{equation}

This well-defined bid function\footnote{Technically, we need to add one more condition on the weights functions: they are still defined in some arbitrarily small- but positive- neighborhood above $\maxbid$, to be able to evaluate the bid-smooth function as a limit from above.}  will be shown to have Jacobian that is positive definite, and as such it yields a unique equilibrium under the constructed proxy game.  The definition of the \textit{bid-smooth mechanism} is: for input bids $\bids$, output the proportional weights allocations as calculated from weights returned from the unique equilibrium of the proxy game parameterized by $\strats^{\delta}$ and $\bids$.

\begin{lemma}
\label{lem:biddeltadef}
For $\wali^+>0$,
\begin{enumerate}
\item  we have that:
\begin{itemize}
\item $\strati^{\delta}(\wali^+,\walsmi) = \strati(\wali^+,\walsmi)$
\end{itemize}
\item and that:
\begin{itemize}
\item $\frac{\partial\strati^{\delta}}{\partial\wali}(\wali^+,\walsmi) = \frac{\partial\strati}{\partial\wali}(\wali^+,\walsmi)$
\item $\frac{\partial\strati^{\delta}}{\partial \wali[j]}(\wali^+,\walsmi) = \frac{\partial\strati}{\partial \wali[j]}(\wali^+,\walsmi)$
\end{itemize}


\item then the only difference between the two bid functions occurs where $\strati^{\delta}$ ``fixes" the discontinuity of $\strati$ being not well-defined at $\wali^0 = 0$.  Instead we have:
\begin{enumerate}
\item $\strati^{\delta}(0,\walsmi) = 0$
\item $\frac{\partial\strati^{\delta}}{\partial\wali}(0,\walsmi) = \frac{\vali'(0)}{2}> 0$
\item $\frac{\partial\strati^{\delta}}{\partial \wali[j]}(0,\walsmi) = 0$
\end{enumerate}
\end{enumerate}

\end{lemma}
\begin{proof}
At all inputs $\wali^+>0$ and all $\walsmi$, the original $\strati$ function is well-defined and continuous and twice-differentiable.  Therefore evaluation in the limit of $\wali^++\delta$ as $\delta\rightarrow 0$ in the $\strati^{\delta}$ function, and direct evaluation in $\strati$, give equal output and equal derivatives.

However by defining evaluation-in-the-limit within the bid function $\strati^{\delta}$ itself, we get % continuity resulting in 
a function and partials well-defined at $\wali^0=0$.  By evaluation:

start by assuming ($\wali^0+\delta) =\delta> 0, \delta\rightarrow 0$, which implies $\alloci(\delta,\walsmi) > 0$.  The integral term in the bid function is upper-bounded by $\alloci(\delta,\walsmi)\cdot\vali(\delta)$, so the entire bid function is lower-bounded by 0 (for all $\delta$ as we converge in the limit).

Trivially bids are upper bounded by values.  So it must be that as $\delta\rightarrow 0$, we have $\strati^{\delta}\rightarrow \left[0,\vali(\delta)\right]$.

By assumptions on weights functions, as $(\wali^0+\delta)=\delta\rightarrow 0 $ it is also that $\vali(\delta)\rightarrow 0$.  Then in fact $\strati^{\delta}\rightarrow 0$.  We conclude (3a), that by definition, $\strati^{\delta}(0,\walsmi) = 0$ for all $\walsmi$.

To analyze the partials at $\wali^0=0$, we use the (multi-variable version of the) calculus technical definition of the derivative function: $\frac{df(x)}{dx} \vcentcolon= \lim_{z\rightarrow 0} \frac{f(x+z)-f(x)}{z}$.
\begin{align*}
\frac{\partial\strati^{\delta}}{\partial\wali}(0,\walsmi) &= \lim_{z\rightarrow 0} \frac{\strati^{\delta}(0+z,\walsmi)-\strati^{\delta}(0,\walsmi)}{z}\\
&= \lim_{z\rightarrow 0} \frac{\strati^{\delta}(z,\walsmi)-0}{z} \text{ (by (3a) of this lemma)}\\
&= \lim_{z\rightarrow 0} \frac{\frac{\partial\strati^{\delta}}{\partial\wali}(z,\walsmi)}{1} \text{ (by L'Hopital)}\\
&= \lim_{z\rightarrow 0} \frac{\partial\strati}{\partial\wali}(z,\walsmi) \text{ (by (2), it is the partial of the original bid function)} \\
&= \frac{\vali'(0)}{2}\geq 0 \text{ (by Lemma~\ref{lem:bidpartlimits} below)}\\
\frac{\partial\strati^{\delta}}{\partial\wali[j]}(0,\walsmi) &= \lim_{z\rightarrow 0}\frac{\strati^{\delta}(0,\wali[j]+z,\wals_{-i,j})-\strati^{\delta}(0,\walsmi)}{z}\\
&= \lim_{z\rightarrow 0}\frac{0-0}{z} = 0 \text{ (by (3a))}
\end{align*}
\end{proof}



\begin{lemma}
\label{lem:bidpartlimits}
Assume the weights functions have $\wali(0) = 0$ for all $i$.  Then the bid partial functions calculated in equations~\eqref{eqn:partialsame} and~\eqref{eqn:partialcross} are not well defined due to the $\frac{1}{\wali}$ terms that appear.  Evaluating these partials instead in the limit $\wali\rightarrow 0$ yields
\begin{align*}
\frac{\partial \bidi}{\partial \wali}(\wals) &\geq 0\\
\frac{\partial \bidi}{\partial \wali[j]}(\wals)&=0
\end{align*}
\end{lemma}
\begin{proof}
\ajc{This is in a lemma/proof block for now but if used will get moved to the section of the appendix where we calculate the bid partials in the first place.}

For the partial of $\strati$ with respect to its own variable $\wali$:
\begin{align*}
\lim_{\wali\rightarrow 0}\frac{\partial \bidi}{\partial \wali}(\wals)&=\lim_{\wali\rightarrow 0}\left[\int_0^{\wali} \vali'(z)\frac{1}{\wali}\frac{z}{\sum_k \wali[k]-\wali+z}\cdot\left(\frac{\sum_k \wali[k] }{\wali}-1\right)dz\right]\\
&=\lim_{\wali\rightarrow 0}\frac{\left[\int_0^{\wali} \vali'(z)\frac{z}{\sum_k \wali[k]-\wali+z}\cdot\left(\sum_k \wali[k] - \wali\right)dz\right]}{\wali^2}\\
& = \lim_{\wali\rightarrow 0}\frac{\vali'(\wali)\left(\frac{\wali}{\sum_k \wali[k]}\right)\cdot\left(\sum_k \wali[k]-\wali\right)}{2\wali}\\
&= \frac{\vali'(0)}{2}\\
&\geq 0
\end{align*}
where moving from the second line to the third invokes L'Hopital's rule, and the reduction in terms moving to the fourth line requires $\sum_k \wali[k]-\wali> 0$ (which further suggests that it is necessary to add a dummy-loss weight to the proportional weights social choice function, which can always be set to 0 tactically).

With the same assumption that $\sum_k\wali[k]-\wali > 0$, for the cross-derivative:
\begin{align*}
\lim_{\wali\rightarrow 0}\frac{\partial \bidi}{\partial \wali[j]}(\wals)&=\lim_{\wali\rightarrow 0}\left[\int_0^{\wali} \vali'(z)\frac{1}{\wali}\frac{z}{\left(\sum_k \wali[k]-\wali+z\right)}\cdot\frac{z(\wali-z)}{\left(\sum_k \wali[k]-\wali+z\right)}dz\right]\\
&=\lim_{\wali\rightarrow 0}\frac{\left[\int_0^{\wali} \vali'(z)\frac{z(\wali-z)}{\left(\sum_k \wali[k]-\wali+z\right)^2}dz\right]}{\wali}\\
&=\lim_{\wali\rightarrow 0}\left[\int_0^{\wali} \vali'(z)\frac{z}{\left(\sum_k \wali[k]-\wali+z\right)^2}dz+\frac{\int_0^{\wali} \vali'(z)\frac{-z^2}{\left(\sum_k \wali[k]-\wali+z\right)^2}dz}{\wali}\right]\\
& = 0+\lim_{\wali\rightarrow 0}\frac{\vali'(\wali)\left(\frac{-\wali^2}{\sum_k \wali[k]}\right)}{1}\\
&=0
\end{align*}
The cross-derivative calculation is slightly more complicated because the $\wali$ term appears both as the upper end point of the integral, and within the integral.
\end{proof}



\begin{corollary}
We extend Theorem~\ref{thm:psdunique} for weights function $\wali(0) = 0$ and the {\em bid-smooth} function $\strati^{\delta}$: it has strictly positive definite Jacobian everywhere on its domain.
\end{corollary}
\begin{proof}
The proof of Theorem~\ref{thm:psdunique} now goes through with one extra intermediate step:

for any dimension realized as $\vali = \wali = 0$, Lemma~\ref{lem:biddeltadef} shows that its row in the Jacobian has positive element in the diagonal and all other elements 0, from:
\begin{itemize}
\item $\frac{\partial\strati^{\delta}}{\partial\wali}(\wali^+,\walsmi) > 0$
\item $\frac{\partial\strati^{\delta}}{\partial \wali[j]}(\wali^+,\walsmi) = 0$
\end{itemize}
Then from this structure, the Jacobian is positive definite if and only if its minor having removed row-and-column $i$ is positive definite.

Reducing the matrix to a minor for all such $j$ with $\wali[j] -0$ leaves us with a matrix subject to the rest of the proof of Theorem~\ref{thm:psdunique}, showing it to be positive definite.

\ajc{actually I think we improved the modularity of the theorem~\ref{thm:psdunique} result and the correct reference here at the end is to the characterization on $H$ matrices.  but I think the idea of this proof is understandable}
\end{proof}

\begin{lemma}
For all true values $\vals$, for all equilibria resulting from the bid-smooth mechanism, agents with $\wali =0$ use the bid function as $\strati(0) = 0$.
\end{lemma}

\begin{proof}
\ajc{Note: with well-defined mechanism, we can finally argue that equilibrium implies a well-defined bid function.

this is a bit hand-wavy, it might need to be cleaned up or have a gap filled:}

Consider agent $i$ with $\vali = \wali = 0$ who considers bidding something other than 0 in equilibrium.

The mechanism is using a bid-smooth function to do the inversion from bids to weights with the following property $\strati = 0$ if and only if $\wali = 0$.

We can see this from Lemma~\ref{lem:biddeltadef}: for every $\walsmi$, $\strati = 0$ if $\wali = 0$, and because the partials $\frac{\partial\strati^{\delta}}{\partial\wali}(\wali^+,\walsmi) > 0$ are strictly greater than,  $\strati > 0$ if $\wali > 0$.

Under the mechanism, calculated $\wali > 0$ gives allocation $\alloci > 0$, which makes bidding 0 a strictly dominant strategy for any agent with $\vali = \wali = 0$.
\end{proof}

\begin{corollary}
For values $\vals\in\left[0,\maxbid\right]$ and weights functions with $\wali(0) = 0$, the {\em bid-smooth mechanism} implements the proportional weights social choice function in Nash equilibrium.
\end{corollary}
\begin{proof}
The result parallels Theorem~\ref{thm:themainresult} in Section~\ref{s:nasheq}, and follows from the results in this Appendix section.
\end{proof}



%However we note the following.

\ajc{the following lemma is not necessarily correct, and even to the extent that it is correct, it is ``deprecated." Specifically note that I was unable to prove the part of the claim about how equilibrium implies that $\strati(0) = 0$ - the analysis ran into a circle.  Equilibrium depends on the mechanism which is an algorithm defined by a bid function which was undefined and which we could not use properties of equilibrium to fix.  More intuition inline below }


\begin{lemma}
In the case where $\wali(0) = 0$, the bid function in weights space is undefined at $\wali = 0$.  Appending the bid function with $\strati(0) = 0$ is
 consistent with evaluating the function in the limit $\wali\rightarrow 0$.

Then further, for {\em any} mechanism $\mathcal{M}$ implementing the proportional weights social choice function as a continuous function of the input $\bids$, 
%Further, % in the case where $\wali(0) > 0$, 
bidding $\strati=0$ is the uniquely optimal strategy for an agent with $\vali = \wali = 0$ in Nash equilibrium.  This claim also holds in the case of $\wali(0) > 0$.
\end{lemma}

\begin{proof}[Proof Attempt!]

\ajc{ be sure to see the comment before the lemma statement before reading this proof to understand context.}
To handle the case $\wali(0) = 0$, we start by assuming $\wali > 0, \wali\rightarrow 0$, which implies $\alloci > 0$.  The integral term in the bid function is upper-bounded by $\alloci(\wals)\cdot\vali(\wali)$, so the entire bid function is lower-bounded by 0.

By assumptions on weights functions, as $\wali\rightarrow 0 $ it is also that $\vali\rightarrow 0$.  Trivially bids are upper bounded by values.

So it must be that as $\wali\rightarrow 0$, we have $\strati\rightarrow \left[0,\vali\right]$, and in fact $\strati\rightarrow 0$.

%Any mechanism $\mathcal{M}$ implementing the social choice function on the true values must give each agent the correct proportional weights allocation.  Specifically, the weights and allocation are fixed

We now consider the necessity of $\strati(0) =0$ under any Nash equilibrium of 

\ajc{as far as I can tell, there is a gap here. we would need to argue that for every value profile containing a 0-value-agent, for every Nash equilibrium of the specific mechanism as described in Section 4 (utility functions parameterized by the values, weakly undominated actions are bids), the 0-value-agent bids 0; a sufficient contrapostive-type claim would be that every positive bid (for any value profile) receives strictly positive allocation.

Specifically note: it would be ``begging the question" to assume properties of the unique equilibrium that we sequentially prove on top of this lemma to argue that b(0) must be 0 ``in equilibrium."  This includes, it would beg the question to assume (at this point) that we have any of a set of mechanisms all of which implement the social choice function; for the mechanism is section 4, that is something we are trying to prove through its unique equilibrium + mechanism => social choice function.}

If instead $\wali(0) > 0$, then agent $i$ always has positive weight and always has positive allocation according to the social choice function.  Then for any mechanism implementing the social choice function on any Nash played by the agents given the mechanism, we get the following.

When $\vali = 0$, bidding anything other than 0 wins with some positive probability and makes a positive payment with some positive probability, while value from winning is 0.  Then utility is strictly negative for all positive bids and 0 when bidding 0, which is strictly dominant.
\end{proof}




==> a_psdunique.tex <==
\section{Proof of Sufficiency of Positive Definiteness}
\label{a:psdunique}

The following proof of Theorem~\ref{thm:psdunique} is adapted from
\citet{GN-65} and included for completeness.



\begin{proof}[of Theorem~\ref{thm:psdunique}]
By contradiction, suppose the Jacobian is positive definite but there are two valuations vectors $\vals^0$ and $\vals^1$ that map to the same bid vector $\bids^*$.
Let vector $\vals^{\lambda}$ be a linear combination as

$$\vals^\lambda=\vals^0+\lambda(\vals^1-\vals^0)$$
Define function $$f(\lambda)=\left[\strats(\vals^\lambda)\right]^\top\cdot (\vals^1-\vals^0)$$
Since $\bids^* = \strats(\vals^0)=\strats(\vals^1)$, we have 
$f(0)=f(1)$.
Function $f$ is continuously differentiable, so there exists $\lambda^*$ such that $$f'(\lambda)\Big|_{\lambda^*}=0$$
Then we get the following:
\begin{eqnarray*}
\left[\frac{\partial \strats  }{\partial \lambda}(\vals^{\lambda^*})\right]^\top\cdot (\vals^1-\vals^0) &=&0
\end{eqnarray*}
\begin{eqnarray*}
\left[\frac{\partial \strati[1]  }{\partial \lambda}(\vals^{\lambda^*}),\frac{\partial \strati[2]  }{\partial \lambda}(\vals^{\lambda^*}),...,\frac{\partial \strati[n]  }{\partial \lambda}(\vals^{\lambda^*})\right]^\top\cdot (\vals^1-\vals^0) &=&0
\end{eqnarray*}
\begin{eqnarray*}
\left[\sum_j\frac{\partial \strati[1]  }{\partial  \val_j^{\lambda}}\cdot \frac{\partial  \val_j^{\lambda}}{\partial \lambda}(\vals^{\lambda^*}),...,\sum_j\frac{\partial \strat_n  }{\partial  \val_j^{\lambda}}\cdot \frac{\partial  \val_j^{\lambda}}{\partial \lambda}(\vals^{\lambda^*})\right]^\top \cdot (\vals^1-\vals^0) &=&0
\end{eqnarray*}
\begin{eqnarray}
\label{eqn:posdef}
(\vals^1-\vals^0)^\top\cdot J_{\strats}(\vals^{\lambda^*}) \cdot (\vals^1-\vals^0) &=&0
\end{eqnarray}
by $\frac{\partial\vali[j]^{\lambda}}{\partial\lambda}(\vals^{\lambda^*}) = (\vali[j]^1-\vali[j]^0)$ and where the $(i,j)$ entry in matrix $J_{\strats}(\vals^{\lambda^*})$ is 
$$\frac{\partial \strat_i  }{\partial  \vali[j]^{\lambda}}(\vals^{\lambda^*})$$
%such that $J_{\bids}$ is realized as the Jacobian matrix of the bid function.  By our assertion, for the set of coordinates of $\vals^0$ and $\vals^1$ that do not coincide equation~(\eqref{eqn:posdef}) has at least one non-trivial solution. However, the coordinates from any solution select a principal minor from $J_{\bids}$ which is positive definite by the statement of the theorem with the determinant bounded away from zero. That means that equation~(\eqref{eqn:posdef}) can only have a trivial solution, which is a contradiction.
%
\noindent such that $J_{\strats}$ is realized as the Jacobian matrix of the bid function evaluated at $\vals^{\lambda^*}$.  By our assertion, $\vals^0$ and $\vals^1$ are distinct such that $(\vals^1-\vals^0)$ is a non-zero vector, and now Equation~(\ref{eqn:posdef}) is seen to contradict the assumption of strict positive definiteness everywhere, by its definition that for pos. def. matrix $M$, it has $\vecbz^{\top} M \vecbz > 0, \forall \vecbz \neq \textbf{0}$.

\end{proof}



==> ss_related_work.tex <==
\paragraph{Related Work.}

%
% comparison to Hartline Taggart
%

This paper is on non-revelation mechanism design as it applies to
online markets.  The goals of this paper -- in providing foundations
for non-revelation mechanism design -- are closest to those of
\citet{HT-16}.  Both papers study iterated environments and the design
of mechanisms welfare that is arbitrarily close to the optimal welfare
under general constraints.  (That paper additionally considers the
objective of maximizing revenue; we additionally consider
implementation of general social choice functions.)  The equilibrium
concept in \citet{HT-16} is Bayes-Nash equilbrium and it is assumed
that agents are short-lived.  These assumptions are not appropropriate
for the design of online markets considered in this paper, where
agents are long-lived and have persistent preferences.

%
% comparison to implementation theory
%

The theoretical questions studied in this paper can be best
interpreted in the context of the literature on non-parametric
implementation theory \citep[for a survey, see][]{jac-01}.  A social
choice rule is a mapping from agent preferences to outcomes.  A
mechanism implements a social choice rule (under a given solution
concept) if the unique outcome of the mechanism that is predicted by
the solution concept is equal to the outcome prescribed by the social
choice rule.  A non-parametric implementation is one that is given by
a single mechanism (for any preferences of the agents).  The
mechanisms identified in the implementation theory literature are
typically given as extensive form games in which agents are required
to take part in some degree of crossreporting, i.e., reporting the
values of the other agents.  This crossreporting makes the resulting
equilibria non-robust and the suggested mechanisms impractical.  In
contrast, this paper's focus on winner-pays-bid mechanisms -- where
agents bids, the mechanism chooses a set of winners, and each winner
pays her reported bid -- naturally excludes such solutions.  

%
% comparison to persuasion
%

Our study of dashboard mechanisms can be compared to the literature on
Bayesian persuasion \citep[e.g.,][]{KG-11,DX-16}.  In our paper and
this literature the principal has more information than the agent and
can signal the agent to alter the agent's beliefs and thus behavior.
In the persuasion literature the agent updates its prior based on the
principal's signal.  The principal's goal is to persuade the agent to
take an action that the principal prefers.  Our work does not assume a
prior and instead allows that there will be multiple rounds and that
an agent will be willing to follow the principal's suggestion in the
short term, and will continue to do so in the long term only if it is
a good strategy.  The specific actions of the agent are not important
in this paper, what is important is that these actions are best
responses to the dashboard and the agent's value can be inferred.

Our work directly relates to specific studies in the literature on the
price of anarchy.  In the bandwidth allocation problem \citet{JT-04}
show that the all-pay proportional bids mechanism is a 4/3
approximation to the optimal welfare for agents with concave value
functions.  Our study of Nash implementation of the proportional
weights social choice function can be adapted to all-pay mechanisms
(from winner-pays-bid mechanisms) and with this adaptation our results
show that for agents with linear value functions there is an all-pay
mechanism that allocates arbitrarily closely to the optimal welfare.

There have been extensive studies of the price of anarchy of ad
auctions, e.g., on the Google search
engine \citep{LT-10,CKKK-11,ST-13}.  A conclusion of these studies is
that in standard models of equilibrium the industry-standard
generalized second price auction can have welfare that is a constant
factor worse than the optimal welfare.  These auctions can be retrofit
with a bidding dashboard and the agents ranking can be adjusted by a
quality score based on our method for inferring values to produce
welfare optimal outcomes in the sponsored search auction model
with stochastic user clicks (considered, e.g. in \citealp{AN-10}).  The resulting dashboard mechanism is welfare
optimal for persuadable agents (i.e., under our solution concept for
dashboard mechanisms).



